FIND: A Function Description Benchmark for Evaluating Interpretability Methods

Labeling neural network submodules with human-legible descriptions is useful for many downstream tasks: such descriptions can surface failures, guide interventions, and perhaps even explain important model behaviors. To date, most mechanistic descriptions of trained networks have involved small models, narrowly delimited phenomena, and large amounts of human labor. Labeling all human-interpretable sub-computations in models of increasing size and complexity will almost certainly require tools that can generate and validate descriptions automatically. Recently, techniques that use learned models in-the-loop for labeling have begun to gain traction, but methods for evaluating their efficacy are limited and ad-hoc. How should we validate and compare open-ended labeling tools? This paper introduces FIND (Function INterpretation and Description), a benchmark suite for evaluating the building blocks of automated interpretability methods. FIND contains functions that resemble components of trained neural networks, and accompanying descriptions of the kind we seek to generate. The functions span textual and numeric domains, and involve a range of real-world complexities. We evaluate methods that use pretrained language models (LMs) to produce descriptions of function behavior in natural language and code. Additionally, we introduce a new interactive method in which an Automated Interpretability Agent (AIA) generates function descriptions. We find that an AIA, built from an LM with black-box access to functions, can infer function structure, acting as a scientist by forming hypotheses, proposing experiments, and updating descriptions in light of new data. However, AIA descriptions tend to capture global function behavior and miss local details. These results suggest that FIND will be useful for evaluating more sophisticated interpretability methods before they are applied to real-world models.

==> figlatex/entities_table_double.tex <==
% \small
% \begin{longtable}{lcc}
% \caption{Atomic entities and Vicuna scores for Synthetic Neural Modules}\\
% \toprule
% \textbf{Entity} & \textbf{Same Entity Score} & \textbf{Random Entity Score} \\ \midrule
% \endfirsthead
% \multicolumn{3}{c}{{\tablename\ \thetable{} -- continued from previous page}} \\ 
% \midrule
% \textbf{Entity} & \textbf{Same Entity Score} & \textbf{Random Entity Score} \\ \midrule
% \endhead
\small
\setlength{\tabcolsep}{5pt} 
\begin{longtable}{lcc cc}
\caption{Atomic entities and Vicuna scores for Synthetic Neural Modules}\\
\toprule
 & \multicolumn{2}{c}{\textbf{Pretrained Vicuna}} & \multicolumn{2}{c}{\textbf{Vicuna-Module}}\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 \textbf{Entity} & \textbf{same entity} & \textbf{random entity} & \textbf{same entity} & \textbf{random entity} \\ 
\midrule
\endfirsthead
\multicolumn{5}{c}{{\tablename\ \thetable{} -- continued from previous page}} \\ 
\midrule
 & \multicolumn{2}{c}{\textbf{Pretrained Vicuna}} & \multicolumn{2}{c}{\textbf{Vicuna-Module}}\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 \textbf{Entity} & \textbf{same entity} & \textbf{random entity} & \textbf{same entity} & \textbf{random entity} \\ 
\midrule
\endhead
sport organizations & 0.9959 & 0.1125 & 0.7973 & 0.0001 \\ 
corporations & 0.9684 & 0.0532 & 0.9996 & 0.0001 \\ 
elections & 0.6703 & 0.0123 & 0.9967 & 0.0007 \\ 
musical works & 0.9785 & 0.1100 & 0.9986 & 0.1001 \\ 
films & 0.9917 & 0.0225 & 0.9134 & 0.0001 \\ 
climate & 0.8098 & 0.0091 & 0.9994 & 0.0001 \\ 
computer hardware & 0.9719 & 0.0038 & 0.7680 & 0.0001 \\ 
physics & 0.9916 & 0.0211 & 0.9995 & 0.0001 \\ 
religions and beliefs & 0.8985 & 0.0132 & 0.7999 & 0.0001 \\ 
law and justice & 0.9952 & 0.1045 & 0.9992 & 0.0001 \\ 
transport & 0.7865 & 0.1295 & 0.8966 & 0.0997 \\ 
education & 0.7831 & 0.1221 & 0.6190 & 0.0001 \\ 
politics & 0.5083 & 0.0295 & 0.8341 & 0.0001 \\ 
works of fiction & 0.9708 & 0.0874 & 0.9982 & 0.0060 \\ 
games and leisure activities & 0.7633 & 0.1361 & 0.9289 & 0.0001 \\ 
biology & 0.9938 & 0.1682 & 0.9997 & 0.1041 \\ 
mathematics & 0.9934 & 0.0196 & 0.9926 & 0.0008 \\ 
geology & 0.9931 & 0.0437 & 0.9993 & 0.0003 \\ 
government and state & 0.6445 & 0.0669 & 0.6352 & 0.0008 \\ 
food and eating & 0.8545 & 0.1013 & 0.8898 & 0.0508 \\ 
air transport & 0.7626 & 0.0112 & 0.9159 & 0.0001 \\ 
road transport & 0.7874 & 0.0268 & 0.9995 & 0.0004 \\ 
rail transport & 0.6717 & 0.0012 & 0.9063 & 0.0000 \\ 
cycling & 0.8464 & 0.0107 & 0.9986 & 0.0208 \\ 
the New York Times & 0.7032 & 0.1633 & 0.9963 & 0.0001 \\ 
aircraft & 0.7367 & 0.0035 & 0.9449 & 0.0001 \\ 
bodies of water & 0.9919 & 0.0940 & 0.9940 & 0.0002 \\ 
mineralogy & 0.9840 & 0.0539 & 0.6998 & 0.0001 \\ 
occupations & 0.9763 & 0.1776 & 0.9371 & 0.0953 \\ 
professional wrestling & 0.8720 & 0.0036 & 0.9997 & 0.0002 \\ 
quantity indicating a percentage & 0.9957 & 0.1476 & 0.9960 & 0.0004 \\ 
plays & 0.5460 & 0.1495 & 0.9958 & 0.0002 \\ 
horses & 0.9641 & 0.0045 & 0.9997 & 0.0001 \\ 
photography & 0.9773 & 0.0263 & 0.9995 & 0.0001 \\ 
music & 0.9646 & 0.0379 & 0.9848 & 0.0001 \\ 
fashion & 0.8981 & 0.1535 & 0.9909 & 0.1237 \\ 
chess & 0.7004 & 0.0042 & 0.6854 & 0.0002 \\ 
racket sports & 0.8277 & 0.1293 & 0.8580 & 0.0998 \\ 
art & 0.9913 & 0.4575 & 0.9650 & 0.0001 \\ 
disasters & 0.6871 & 0.0219 & 0.8778 & 0.0005 \\ 
spacecraft & 0.9146 & 0.0182 & 0.9905 & 0.0001 \\ 
video games & 0.9912 & 0.0348 & 0.9991 & 0.0760 \\ 
the relationship of an element to its class & 0.8927 & 0.7081 & 0.9368 & 0.0157 \\ 
basketball & 0.7669 & 0.0087 & 0.9997 & 0.0001 \\ 
winter sports & 0.9844 & 0.0020 & 0.9996 & 0.0000 \\ 
American football & 0.8486 & 0.0365 & 0.9997 & 0.0013 \\ 
golf & 0.9250 & 0.0264 & 0.9996 & 0.0002 \\ 
baseball & 0.8925 & 0.0061 & 0.9997 & 0.0003 \\ 
ice hockey & 0.6633 & 0.0030 & 0.9965 & 0.1002 \\ 
women and feminism & 0.8189 & 0.1201 & 0.9991 & 0.0470 \\ 
lighthouses & 0.4934 & 0.0099 & 0.8476 & 0.0001 \\ 
tennis & 0.8036 & 0.0079 & 0.8921 & 0.0001 \\ 
water sports & 0.9583 & 0.0143 & 0.9996 & 0.0001 \\ 
comics & 0.6374 & 0.0117 & 0.7982 & 0.0000 \\ 
algorithms & 0.8007 & 0.0215 & 0.9996 & 0.0007 \\ 
tourism & 0.6905 & 0.1859 & 0.8635 & 0.0009 \\ 
bridges & 0.6850 & 0.0125 & 0.9988 & 0.0001 \\ 
books & 0.7735 & 0.1113 & 0.9978 & 0.0001 \\ 
linguistics & 0.9951 & 0.4636 & 0.9991 & 0.0006 \\ 
utilization and ownership & 0.4016 & 0.2057 & 0.9513 & 0.0000 \\ 
online communities & 0.8894 & 0.0843 & 0.6305 & 0.0000 \\ 
television & 0.8507 & 0.0228 & 0.9888 & 0.0002 \\ 
astronomy & 0.9952 & 0.0540 & 0.9636 & 0.0038 \\ 
disability & 0.6367 & 0.0234 & 0.9995 & 0.0000 \\ 
proteins & 0.3989 & 0.0718 & 0.9581 & 0.0005 \\ 
human anatomy & 0.9658 & 0.0526 & 0.9997 & 0.0001 \\ 
gymnastics & 0.7507 & 0.0265 & 0.7882 & 0.0001 \\ 
architecture & 0.7997 & 0.0552 & 0.8004 & 0.0001 \\ 
sculpture & 0.7950 & 0.0305 & 0.6187 & 0.0001 \\ 
archaeology & 0.8363 & 0.0830 & 0.8206 & 0.0001 \\ 
theater & 0.8991 & 0.1045 & 0.9991 & 0.0002 \\ 
dams & 0.7765 & 0.0118 & 0.9996 & 0.0002 \\ 
birds and ornithology & 0.9934 & 0.0695 & 0.9995 & 0.0002 \\ 
computing & 0.9881 & 0.3017 & 0.9990 & 0.1199 \\ 
time and duration & 0.6986 & 0.0518 & 0.9913 & 0.0423 \\ 
age & 0.8319 & 0.0400 & 0.9994 & 0.0001 \\ 
weapons and military equipment & 0.8205 & 0.0032 & 0.8966 & 0.0000 \\ 
ratios and proportions & 0.4462 & 0.1546 & 0.3503 & 0.0707 \\ 
typefaces and typography & 0.9114 & 0.0942 & 0.9984 & 0.0019 \\ 
burials graves and memorials & 0.8778 & 0.0101 & 0.9997 & 0.0001 \\ 
processes and manufacturing & 0.6454 & 0.0585 & 0.9778 & 0.0001 \\ 
paleontology & 0.9337 & 0.0544 & 0.9823 & 0.0237 \\ 
banking & 0.9224 & 0.0337 & 0.9997 & 0.0570 \\ 
lakes & 0.5523 & 0.0597 & 0.5190 & 0.0963 \\ 
natural science & 0.9700 & 0.3590 & 0.9965 & 0.0335 \\ 
geography & 0.9814 & 0.0393 & 0.9994 & 0.0004 \\ 
insects and entomology & 0.8974 & 0.0333 & 0.9941 & 0.0001 \\ 
philosophy & 0.9914 & 0.1678 & 0.9995 & 0.0001 \\ 
poetry & 0.9914 & 0.0709 & 0.9997 & 0.0040 \\ 
encyclopedias & 0.6422 & 0.3503 & 0.9036 & 0.0009 \\ 
television shows & 0.9136 & 0.0955 & 0.9699 & 0.0950 \\ 
awards prizes and honours & 0.9968 & 0.1588 & 0.9334 & 0.0006 \\ 
the Middle Ages & 0.8710 & 0.0530 & 0.8440 & 0.0001 \\ 
plants and botany & 0.9938 & 0.1890 & 0.9915 & 0.1000 \\ 
marine biology & 0.9958 & 0.0587 & 0.9994 & 0.1000 \\ 
color & 0.7804 & 0.0798 & 0.9989 & 0.0001 \\ 
airports & 0.7118 & 0.0032 & 0.9997 & 0.0001 \\ 
science & 0.9464 & 0.2842 & 0.9795 & 0.0177 \\ 
anime and manga & 0.9689 & 0.0941 & 0.9996 & 0.0000 \\ 
Christianity & 0.9880 & 0.0146 & 0.9997 & 0.0003 \\ 
Buddhism & 0.9931 & 0.0022 & 0.9997 & 0.0010 \\ 
Greek mythology & 0.9493 & 0.0127 & 0.9995 & 0.0001 \\ 
Judaism and the Jewish people & 0.9650 & 0.0122 & 0.9996 & 0.0000 \\ 
music genres & 0.9873 & 0.1441 & 0.9991 & 0.0004 \\ 
fictional characters & 0.8917 & 0.1441 & 0.9995 & 0.0999 \\ 
rap and hip hop & 0.6931 & 0.0555 & 0.9799 & 0.1106 \\ 
Islam & 0.9486 & 0.0163 & 0.9997 & 0.0002 \\ 
The Walt Disney Company & 0.9365 & 0.0047 & 0.9991 & 0.0000 \\ 
agriculture & 0.9816 & 0.1044 & 0.9022 & 0.1000 \\ 
hiking & 0.3838 & 0.0176 & 0.8673 & 0.0001 \\ 
New York City & 0.9687 & 0.1131 & 0.9993 & 0.0909 \\ 
gardens & 0.8955 & 0.0929 & 0.9979 & 0.0454 \\ 
personality traits & 0.8791 & 0.1725 & 0.9986 & 0.0001 \\ 
camping & 0.7282 & 0.0651 & 0.8878 & 0.0953 \\ 
gender & 0.5555 & 0.0488 & 0.9995 & 0.0001 \\ 
cemeteries and graves & 0.9843 & 0.0272 & 0.9997 & 0.0001 \\ 
London & 0.9541 & 0.1048 & 0.9991 & 0.0147 \\ 
Los Angeles & 0.9489 & 0.0424 & 0.9993 & 0.0003 \\ 
Chicago & 0.9586 & 0.0469 & 0.9994 & 0.0001 \\ 
Paris & 0.7892 & 0.0169 & 0.9017 & 0.0001 \\ 
Berlin & 0.9228 & 0.0522 & 0.8216 & 0.0396 \\ 
sailing & 0.8972 & 0.0015 & 0.9995 & 0.0103 \\ 
swimming & 0.9009 & 0.0152 & 0.9996 & 0.0001 \\ 
the Holocaust & 0.7882 & 0.0070 & 0.9257 & 0.0019 \\ 
arachnids and arachnology & 0.7985 & 0.1284 & 0.8606 & 0.0001 \\ 
musical instruments & 0.9971 & 0.0420 & 0.9990 & 0.0001 \\ 
meteorology & 0.9256 & 0.0108 & 0.9995 & 0.0001 \\ 
disease & 0.7874 & 0.0096 & 0.9996 & 0.0000 \\ 
Ireland & 0.7840 & 0.0200 & 0.9968 & 0.0007 \\ 
libraries & 0.6125 & 0.1224 & 0.9990 & 0.0001 \\ 
museums & 0.8481 & 0.0581 & 0.8889 & 0.0001 \\ 
journalism & 0.8834 & 0.0205 & 0.9205 & 0.0001 \\ 
buildings & 0.7952 & 0.1530 & 0.8123 & 0.0078 \\ 
cryptocurrencies & 0.9511 & 0.0008 & 0.9996 & 0.0001 \\ 
events and news & 0.7247 & 0.2294 & 0.7649 & 0.0943 \\ 
Louisiana & 0.7446 & 0.0119 & 0.9991 & 0.0001 \\ 
revolutions & 0.6227 & 0.0755 & 0.9927 & 0.0522 \\ 
mines and mining & 0.9179 & 0.0393 & 0.9790 & 0.0007 \\ 
Switzerland & 0.9468 & 0.0497 & 0.9960 & 0.0001 \\ 
World War II & 0.9858 & 0.0643 & 0.9993 & 0.1001 \\ 
\midrule
\textbf{Average} & \textbf{0.8462} & \textbf{0.0787} & \textbf{0.9389} & 
\textbf{0.0185}   \\
\bottomrule
\label{tab:all_entities_new}
\end{longtable}

==> figlatex/find_math_table.tex <==

\begin{wraptable}{r}{.4\linewidth}
  \caption{ \textbf{\findfunctions} mathematical functions}
  \vspace{2mm}
  \label{tab:mathfunctions}
  \centering
  {\small
  \begin{tabular}{lr}  
    \toprule
    \multicolumn{2}{c}{\textbf{Atomic Functions}} \\
    \midrule
    \multicolumn{2}{c}{\textbf{Algebraic Functions}}\\
    Linear & $mx + b$ \\
    Polynomial & $a_0 + a_1x + a_2x^2 + \dots + a_nx^n$ \\
    Absolute & $a|x| + b$ \\
    Rational & $\frac{P(x)}{Q(x)}$ \\
    Reciprocal & $\frac{1}{ax}$ \\
    \midrule
    \multicolumn{2}{c}{\textbf{Periodic Functions}}\\
    Sin & $a\sin\left(\frac{2\pi}{b}(x-c)\right) + d$ \\
    Cos & $a\cos\left(\frac{2\pi}{b}(x-c)\right) + d$ \\
    Tan & $a\tan\left(\frac{2\pi}{b}(x-c)\right) + d$ \\
    \midrule
    \multicolumn{2}{c}{\textbf{Exponential and Logarithmic Functions}}\\
    Exponential & $ae^{bx}$ \\
    Logarithm & $a\log_b(x) + c$ \\
    \midrule
    \multicolumn{2}{c}{\textbf{Piecewise Functions}}\\
    Step & $aH(x - s) + b$ \\
    ReLU & $a\max(0, x) + b$ \\
    Rectangle & $1 if |x| \leq \frac{w}{2}$ \\
    Square wave & $sgn(\sin\left(\frac{2\pi}{T}(x-\phi)\right))$ \\
    \midrule
    \multicolumn{2}{c}{\textbf{Special Functions}}\\
    Sigmoid & $a\left(\frac{1}{1 + e^{-x/t}}\right) + b$ \\
    Tanh & $a\tanh\left(\frac{2\pi}{b}(x-c)\right) + d$ \\
    Gaussian & $\frac{1}{\sigma\sqrt{2\pi}}e^{-\frac{(x-\mu)^2}{2\sigma^2}}$ \\
    Student t & $\frac{\Gamma((\nu+1)/2)}{\sqrt{\nu\pi}\Gamma(\nu/2)}(1 + x^2/\nu)^{-(\nu+1)/2}$ \\
    Power & $ax^p + b$ \\
    \midrule
    Constant & $c$\\
    \bottomrule
  \end{tabular}
  }
\end{wraptable}

==> figlatex/math_examples.tex <==
\begin{figure}[b!]
    \centering
\includegraphics[width=\textwidth]{figures/placeholder_math.png}
    \caption{We should also have an example figure of each of the types of complexity that can be added to a math function.}
    \label{fig:math_examples}
\end{figure}

==> figlatex/relations_accuracies.tex <==
\begin{table}
\centering
\caption{Vicuna factual accuracies implementing relation modules}
\begin{tabular}{@{}lcc@{}}
\toprule
& \textbf{Atomic relations} & \textbf{Relations with domain corruptions}  \\
\midrule
\textbf{Pretrained Vicuna} & 0.96 & 0.67 \\
\textbf{Vicuna-Module} & 0.97 & 0.97 \\
\bottomrule
\end{tabular}
\label{tab:relations_accuracies}
\end{table}


==> figlatex/relations_corrupted.tex <==
\small
\begin{table}
\small
\centering
\caption{Factual relations with domain corruptions}
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Input} & \textbf{Output with domain corruption} <corruption $1$, corruption $2$> 
\\ \midrule

country & capital of the country EXCEPT if the country is in <Asia, S. America> \\

city & country where the city is located EXCEPT if the city is in <Mexico, The U.S.> \\

head of state & country where head of state EXCEPT if the head of state is a <man, woman> \\

monument & country where located EXCEPT if the monument is in <New York City, France> \\

monument & continent where located EXCEPT if the monument is in <S. America, Australia> \\

city in the U.S. & state where the city is located EXCEPT if the city is in <California, Texas> \\

country & official language of the country EXCEPT if the country is in <N. America, S. America> \\

well-known person & occupation of the person EXCEPT if the person is a <woman, man> \\

name of a person & most likely gender of the person EXCEPT if the name begins with <T, S> \\

country & continent where the country is located EXCEPT if the country is in <Asia, Europe> \\

opera & composer of the opera EXCEPT if the opera is in <Italian, German> \\

title of a book & author of the book EXCEPT if the book was written <before $1900$, after $1900$> \\

country & another country on its border EXCEPT if the country is in <Africa, N. America> \\

politician & political party of the politician EXCEPT if the politician is a <man, woman> \\

river & continent where the river is located EXCEPT if the continent is <Africa, Europe> \\

city & time zone of the city EXCEPT if the city is in <N. America, Asia> \\

opera & language of the opera EXCEPT if the opera is in <English, Italian> \\

animal &  main food source of the animal EXCEPT if the animal is a <carnivore, herbivore> \\

animal & typical habitat of the animal EXCEPT if the animal lives on <land, in the ocean> \\

gemstone & color of the gemstone EXCEPT if the gemstone is <red, blue> \\

\bottomrule
\end{tabular}
\label{tab:relations_corrupted}
\end{table}


==> figlatex/relations_uncorrupted.tex <==
\small
\begin{table}
\small
\centering
\caption{Atomic factual relations}
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Input} & \textbf{Output} \\ \midrule

country & capital of the country \\

city & country where the city is located \\

head of state & country where that person was head of state \\

monument & country where the monument is located  \\

monument & continent where the monument is located  \\

city in the U.S. & state where the city is located \\

country & official language of the country  \\

well-known person & occupation of the person \\

name of a person &  most likely gender of the person \\

country & continent where the country is located  \\

opera & composer of the opera  \\

title of a book & author of the book \\

country & another country on its border \\

politician & political party of the politician \\

river & continent where the river is located  \\

city & time zone of the city \\

opera & language of the opera  \\

animal &  main food source of the animal \\

animal & typical habitat of the animal \\

gemstone & color of the gemstone \\

first name & family name of a well-known person with that first name \\

well-known person & person's country of origin \\ 

musical group & musical group's country of origin \\

word & hyperonym of the word \\ 

film & cast member of the film \\

painting & painter of the painting \\

animal & taxonomic class of the amimal \\

well-known person & person's place of birth \\

film & director of the film \\

musical artist & musical genre \\

car model & manufacturer of that car model \\

plant & taxonomic class of the plant \\

artwork & primary material used to create the artwork \\

book & original language of the book \\

planet & number of moons of the planet \\

\bottomrule
\end{tabular}
\label{tab:relations}
\end{table}


==> figlatex/strings_table.tex <==
%make this a wraptable 
\begin{table}
  \caption{Example string functions}
  \centering
  \begin{tabular}{ll}
    \toprule
    \multicolumn{2}{c}{\textbf{Example atomic functions}}   \\
    \midrule
    \verb|shift_last_letter_forward| & apple $\mapsto$ appld  \\
    \verb|replace_substring(a,b)|     & apple $\mapsto$ bpple      \\
    \verb|remove_duplicates| &  apple $\mapsto$ aple      \\
    \midrule
    \multicolumn{2}{c}{\textbf{Example compositions}}   \\
    \midrule
    \verb|reverse(convert_to_uppercase)| & love $\mapsto$ EVOL  \\
    \verb|duplicate_last_letter(shift_last_letter_forward)|  &  love $\mapsto$ lovff    \\
    \verb|count_vowels(concatenate(`cat'))|    & love $\mapsto$ 3      \\
    \bottomrule
  \end{tabular}
  \label{tab:strings_table}
\end{table}


==> figlatex/vicuna_confusionmat_module.tex <==
\begin{figure}[hbt!]
    \centering
\includegraphics[width=\textwidth]{figures/module_vicuna_confusionmat.png}
    \caption{Entity functions implemented using Vicuna respond more strongly to concepts related to their reference entity (diagonal) than to concepts related to other entities (off-diagonal). The value in row $i$ and column $j$ corresponds to the average output of the entity $e_i$ function for 10 inputs associated with entity $e_j$. Each row is normalized using softmax. The prompt template used to instruct Vicuna to implement each function is shown in Section \ref{sec:prompts}.}
    \label{fig:confusionmat}
    \vspace{8cm}
\end{figure}




==> figlatex/vicuna_confusionmat_pretrained.tex <==
\begin{figure}[hbt!]
    \centering
\includegraphics[width=\textwidth]{figures/pretrained_vicuna_confusionmat.png}
    \caption{Entity functions implemented using Vicuna respond more strongly to concepts related to their reference entity (diagonal) than to concepts related to other entities (off-diagonal). The value in row $i$ and column $j$ corresponds to the average output of the entity $e_i$ function for 10 inputs associated with entity $e_j$. Each row is normalized using softmax. The prompt template used to instruct Vicuna to implement each function is shown in Section \ref{sec:prompts}.}
    \label{fig:confusionmat}
    \vspace{8cm}
\end{figure}




==> latex/03_baseline.tex <==
\section{Function interpretation task}
\label{section:interpretation}

\textbf{\findfunctions} can be used to evaluate any \verb|interpreter| system that has the ability to execute Python scripts autonomously at the command line. As a first demonstration, we evaluate several approaches inspired by recent work \citep{hernandez2022natural,bills2023language,singh2023explaining} that use pre-trained language models to perform interpretation.
We run experiments using the OpenAI Python API. A custom plugin equips the \verb|interpreter| model with the command \verb|PYTHON(function.py value)| that it can use to call functions on its own selection of inputs. 
Scripts for reproducing these baselines and complete interpretation dialogues are available in the \textbf{\findfunctions} \href{https://github.com/multimodal-interpretability/FIND}{code repository}.

The \verb|interpreter| is prompted to run experiments on\textbf{ \findfunctions} functions to produce data that it can use to explain function behavior. Prompts for two categories of functions are reproduced below. For all categories of functions, the \verb|interpreter| is prompted to return a natural language description of function behavior (\verb|[DESCRIPTION]|). In categories where corruption can be introduced to part of the function domain (numeric functions and factual relations), the \verb|interpreter| is also prompted to return a description of the domain of the function (\verb|[DOMAIN]|), indicating any subdomain where the function behaves differently. In the mathematical reasoning and strings categories, the \verb|interpreter| is prompted to return code that implements the function (\verb|[CODE]|). Prompts for additional function categories and system prompts are provided in the Appendix.   

\textbf{Prompt for numeric functions:}
\begin{mylisting}{}
Hi, your job is to interpret a function f(x) that is implemented in the {function.py} script. f(x) takes numerical inputs. All you can do is call f(x) on a value of x by running PYTHON({function.py} value). Try to describe the function implemented by f(x) by running experiments on it. You can call 
the function on multiple inputs at a time by running PYTHON({function.py} value1 value2 value3...). 
You can run the function multiple times on the same input. We encourage testing a large range of values before writing a description. You can test values between [-128 and 128]. The output could be 
noisy and your goal is to find a good simple description of f(x) that explains most of the function behavior. f(x) may combine multiple different operations. There may be an interval inside the domain 
where the function behaves differently. If that is the case, describe that interval. Your description of the function should have three parts. First, 
[DESCRIPTION]: Describe what the function is doing in language. 
[DOMAIN]: What is the domain of the function? Is there an interval where the function displays unexpected behavior? What are the numeric bounds of that interval? What is going on there?
[CODE]: Write Python code that approximates the behavior of the function.
\end{mylisting}

\textbf{Prompt for synthetic neural modules (entities):}
\begin{myyellowbox}{}
Hi, your job is to interpret a function f(x) that is implemented in the {function.py} script. f(x) takes word inputs and returns a value between 0 and 1, where a value closer to 1 indicates the association with a particular concept. Your task is to figure out what that concept is. f(x) may be 
selective for more than one concept. If that is the case, describe all concepts that f(x) is selective for. Try to describe the function implemented by f(x) by running experiments on it. We encourage you to test a diverse and random selection of words: spanning many different categories, including both common and obscure words, concrete and abstract words. You can call the function on multiple inputs at a time by running PYTHON({function.py} word1 word2 word3 ...). We encourage running many tests before writing a description. The goal is to find a good simple description of 
f(x) that explains most of the function behavior. Your description of the function should be in the following form. [DESCRIPTION]: Describe what the function is doing in language. 
\end{myyellowbox}

We show complete GPT-4 interpretation dialogues for two example functions in Figure \ref{fig:interpretation}. As the \verb|interpreter| is instructed to run \verb|PYTHON(function.py value)| itself for each function, interpretation occurs without any human input. Even when the final explanation is not fully accurate (see the predicted numeric function in Figure \ref{fig:interpretation}), the conversation history shows a structured interpretation procedure. The \verb|interpreter| makes and tests informed hypotheses about the functions: testing densely spaced points in a specific interval to reveal a ``separating point'' in the behavior of the numeric function, and testing different forms of transportation to determine whether the function is selective for land, sea, or air travel. Once the \verb|interpreter| has gathered sufficient data and produces a final description, the run stops automatically. The Appendix further describes experimental settings.


\input{figlatex/interpretation}

==> latex/10_checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}(See Section 4)
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} See GitHub link in Section \ref{sec:introduction} (and Appendix)
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}See Appendix
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}See Appendix
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}See Appendix.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}{}
  \item Did you mention the license of the assets?
    \answerYes{}See Section \ref{section:neurons} and Appendix.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
